Deterministic vs. Non Deterministic Finite Automata in Automata Processing

Linear-time pattern matching engines have seen promising results using Finite Automata (FA) as their computation model. Among different FA variants, deterministic (DFA) and non-deterministic (NFA) are the most commonly used computation models for FA-based pattern matching engines. Moreover, NFA is the prevalent model in pattern matching engines on spatial architectures. The reasons are: i) DFA size, as in #states, can be exponential compared to equivalent NFA, ii) DFA cannot exploit the massive parallelism available on spatial architectures. This paper performs an empirical study on the #state of minimized DFA and optimized NFA across a diverse set of real-world benchmarks and shows that if distinct DFAs are generated for distinct patterns, #states of minimized DFA are typically equal to their equivalent optimized NFA. However, NFA is more robust in maintaining the low #states for some benchmarks. Thus, the choice of NFA vs. DFA for spatial architecture is less important than the need to generate distinct DFAs for each pattern and support these distinct DFAs' parallel processing. Finally, this paper presents a throughput study for von Neumann's architecture-based (CPU) vs. spatial architecture-based (FPGA) automata processing engines. The study shows that, based on the workload, neither CPU-based automata processing engine nor FPGA-based automata processing engine is the clear winner. If #patterns matched per workload increases, the CPU-based automata processing engine's throughput decreases. On the other hand, the FPGA-based automata processing engine lacks the memory spilling option; hence, it fails to accommodate an entire automata if it does not fit into FPGA's logic fabric. In the best-case scenario, the CPU has a 4.5x speedup over the FPGA, while for some benchmarks, the FPGA has a 32,530x speedup over the CPU.

==> Background.tex <==
\section{Background}
% \subsection{Pattern Matching and DFA, NFA}
% A Finite Automata (FA) is a mathematical model of computation that can be implemented into hardware. DFA and NFA are two variants of FA. The regular expression, which is a commonly used language to represent patterns, can be transformed into an NFA using McNaughton and Yamada algorithm \cite{mcnaughton1960regular}. Moreover, an NFA can be converted to an equivalent DFA using the power-set construction \cite{rabin1959finite}.\\
% Applications such as DNA and protein motif search \cite{roy2015discovering}, filtering ribosomal RNA (rRNA) fragment from metatranscriptomic data \cite{kopylova2012sortmerna} use mesh automata like Hamming and Levenshtein automata to boost their performance. Fortunately, these mesh automata can be represented using NFA or DFA \cite{schulz2002fast}. As a result, high-performance pattern matching engines use either of these two FAs as their computational model.  In Section \ref{sec:state_count_analysis}, we analyze the state count of DFA and NFA for multiple automata benchmarks.
% \begin{figure}[hb]
% \centering
% \begin{subfigure}{0.24\textwidth}
% \centering
% \includegraphics[clip, trim={.5cm .2cm .2cm .4cm},scale=0.55]{Figures/NFADFA/DFA.png}
% \caption{DFA}
% \label{fig:dfa}
% \end{subfigure}
% \begin{subfigure}{0.24\textwidth}
% \centering
% \includegraphics[clip,  trim={1.6cm 0.2cm .2cm 1.1cm},scale=0.55]{Figures/NFADFA/NFA.png}
% \caption{NFA}
% \label{fig:nfa}
% \end{subfigure}
% \caption{FA accepting pattern (a*(b+ba))}
% \label{fig:nfa_dfa}
% \end{figure}
% \subsection{Minimized DFA (mDFA)}
% \label{subsec:mdfa}
% DFA with a large number of states will require a large memory to represent its states, and transitions \cite{kumar2006algorithms}. Fortunately, it is possible to create a minimized DFA (mDFA) from a given DFA in polynomial time \cite{hopcroft2001introduction}. The mDFA for a regular language \emph{L} is the unique DFA with the fewest states that recognize \emph{L}. The mDFA is computed by removing or merging the following two classes of states from a non-minimized DFA:
% \begin{itemize}
%     \item Unreachable States: States in the DFA which cannot be reached from the start state of the DFA for any input pattern.
%     \item Indistinguishable States: States in the DFA that have equivalent transitions for all possible input patterns.  
% \end{itemize}
% Given a DFA, Hopcroft's algorithm \cite{hopcroft1971n} uses the partition-refinement technique to obtain mDFA. In his approach, DFA states are divided into multiple classes such that states belonging to a class are indistinguishable. Consequently, they can be merged into a single state. On the other hand, Brzozowski's algorithm \cite{brzozowski1962canonical} takes NFA as an input and converts it to an mDFA. This algorithm uses \emph{double-reversal} technique as showed in Figure \ref{fig:brzozowski}. The benchmarks we used have their automata in NFA format, and Hopcroft's algorithm doesn't take NFA as an input. As a result, we used Brzozowski's DFA minimization algorithm to generate mDFA for all of our experiments. 
% \begin{figure}[hbt]
% \centering
% \includegraphics[clip, trim={.7cm .7cm .6cm .7cm},scale=0.45]{Figures/dbl_rev.png}
% \caption{Brzozowski's Double-Reversal DFA Minimization}
% \label{fig:brzozowski}
% \end{figure}
\subsection{Optimized NFA}
\label{subsec:opti_NFA}
NFA minimization is a PSPACE-complete problem \cite{jiang1993minimal}. However, there are several algorithms to build smaller NFAs (fewer transitions \cite{hagenah2000computing} and fewer states \cite{ilie2004nfa}). As a result, we use following heuristic to create an optimized NFA:
\begin{itemize}
    \item If multiple states have $equivalent$ $outgoing$ $transitions$ (for all the symbols, they transition into the same states), we merge those states into one state.
\end{itemize}
\subsection{Automata Benchmark}
We use AutomataZoo \cite{wadden2018automatazoo} benchmark suite for all of our experiments. The reason being, benchmarks in AutomataZoo contains larger rule-sets than the ANMLZoo \cite{wadden2016anmlzoo} benchmark suite. Besides, input files in AutomataZoo are curated from real-world data. Hence, to get a pragmatic perception and make the evaluations uniform, we chose benchmarks from AutomataZoo in our study.  However, AutomataZoo doesn't contain any synthetic benchmark. As a result, we used dot-star \cite{yu2013gpu} from ANMLZoo as a representative of the synthetic benchmark class. 

==> void/ActiveRule.tex <==
\section{Active Rule}
\label{subsec:active_rule}
Each automata benchmark consists of multiple rules. The pattern matching applications must process each incoming input pattern through each rule in linear time. However, all the rules of a benchmark might not get triggered equally by each input pattern. Besides, some rules might not get triggered at all. We are referring to the rules triggered by an input pattern as \emph{Active Rules} for that input. There might be some active rules for which the input pattern does not satisfy the condition so that the rule gets executed beyond the start state. To the best of our knowledge, no previous works does this study on the regex-based benchmarks. In this section, we present our study on active rules for the regex-based benchmarks (Snort, Brill, ClamAV) from AutomataZoo.
\begin{enumerate}
    \item For each benchmark, we calculate the frequency of active rules per input cycle. 
    \item Among the active rules, we determine the average percentage of rules that have only one active state. That means, average percentage of active rule that doesn't proceed beyond the start state.
\end{enumerate}
 We perform this study on individual rules of each benchmark. Given an input file, VASim's \cite{wadden2016vasim} \emph{profile} option provides active state histogram for an automata for processing an input pattern. We used AutomataZoo's input file for each benchmark. The Snort input file has \emph{29MB} pattern, Brill has \emph{2MB} pattern, and ClamAV has \emph{64MB} pattern. According to the AutomataZoo paper these inputs are selected from real-world network traffic and malware samples.
\begin{enumerate}
    \item To determine the rule activation frequency while processing an input file, we used VASim's active state histogram, and count the rules that have at least one active state per input cycle. Figure \ref{fig:active_rule_all} presents the rule activation frequency for all three regex-based benchmarks. From Figure \ref{fig:act_rull_snort}, we can see that, \emph{among 2,483 Snort rules, at most 1,041 rules (41.92\%) and at least 12 rules (0.5\%) are active} while processing an input pattern. However, \emph{among 5,946 Brill rules at least 2,339 rules (39.34\%) and at most 5,946 rules (100\%) are active} (Figure \ref{fig:act_rule_brill}). For 4,594 ClamAV rules, the active rule count ranges from 15 (0.33\%) to 271 (5.99\%) (Figure \ref{fig:act_rule_clam}).
    \item From our analysis, we found out that, each individual rule of the regex-based benchmarks, has only one start state. As a result, using VASim's active state histogram, we count the number of rules that have only one active state, which is the start state. Then we used this count to determine among the total active rules what percentage of rules have only one state active. Our analysis shows that among the active rules, Snort has on average 68.98\% and Brill has on average 68.44\% of active rules that don't move past the start state.
\end{enumerate}
\begin{figure*}[h]
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=0.9\linewidth, height=5cm]{Figures/ActiveRules/brillfreqdist.png} 
\caption{Brill}
\label{fig:act_rule_brill}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=0.9\linewidth, height=5cm]{Figures/ActiveRules/snortfreqdist.png}
\caption{Snort}
\label{fig:act_rull_snort}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=0.9\linewidth, height=5cm]{Figures/ActiveRules/sclamfreqdist.png}
\caption{ClamAV}
\label{fig:act_rule_clam}
\end{subfigure}
\caption{Active Rule Count}
\label{fig:active_rule_all}
\end{figure*}

==> void/Experiments.tex <==
\section{Experiments and Evaluations}
This section presents a detailed description of the experiments we performed. Section \ref{subsec:state_comp_ind} and Section \ref{subsec:state_comp_multi} shows the state count experiment on DFA and NFA across multiple benchmark classes. In section \ref{subsec:active_rule},

\subsection{State Count Analysis between NFA and mDFA for Individual Rule}


\label{subsec:multi_state_count_analysis}
\begin{figure*}[h]
\begin{subfigure}{0.33\textwidth}
\begin{subfigure}{\textwidth}
\fbox{\includegraphics[clip,  trim={0.3cm 0.1cm 1.3cm 1.2cm},scale=0.42]{Figures/StateComp/MultipleRules/snort_st_multi.pdf}}{}{}
\caption{Snort}
\label{fig:snort_st_multi}
\end{subfigure}
\begin{subfigure}{\textwidth}
\includegraphics[clip,  trim={0.1cm 0cm 1.3cm 1.1cm},scale=0.3]{Figures/StateComp/MultipleRules/lev_st_multi.pdf}
\caption{Levenshtein}
\label{fig:lev_st_multi}
\end{subfigure}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
\begin{subfigure}{\textwidth}
\includegraphics[clip,  trim={.4cm 0cm 1.2cm 1.2cm},scale=0.4]{Figures/StateComp/MultipleRules/brill_st_multi.pdf}
\caption{Brill}
\label{fig:brill_st_Multi}
\end{subfigure}
\begin{subfigure}{\textwidth}
\includegraphics[clip,  trim={0cm 0cm 1.1cm 1.1cm},scale=0.4]{Figures/StateComp/MultipleRules/ham_st_multi.pdf}
\caption{Hamming}
\label{fig:ham_st_multi}
\end{subfigure}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
\begin{subfigure}{\textwidth}
\includegraphics[clip,  trim={0cm 0cm 1.1cm 1.1cm},scale=0.4]{Figures/StateComp/MultipleRules/clam_st_multi.pdf}
\caption{ClamAV}
\label{fig:clam_st_multi}
\end{subfigure}
\begin{subfigure}{\textwidth}
\includegraphics[clip,  trim={0cm 0cm 1.1cm 1.1cm},scale=0.4]{Figures/StateComp/MultipleRules/dot_st_multi.pdf}
\caption{DotStar}
\label{fig:dot_st_multi}
\end{subfigure}
\end{subfigure}
\caption{State Comparison Between NFA and mDFA}
\label{fig:statecompmulti}
\end{figure*}

\subsection{Hardware Performance}
\label{subsec:hwperf}
\subsection{Random Automata}
\label{subsec:randFA}

==> void/Introduction.tex <==
% \section{Introduction}
% \label{sec:intro}
% Deterministic Finite Automata (DFA) and Non-deterministic Finite Automata (NFA), primary formalisms for the regular expressions, are used alternatively as computational models in many pattern matching engines \cite{sidhu2001fast, rahimi2020grapefruit, gogte2016hare, wang2019hyperscan}. Even though both of these models are functionally equivalent, their structure and transition rules vary \cite{hopcroft2001introduction}. For example, the DFA and NFA presented in Figure \ref{fig:nfa_dfa} both accept the pattern (a*(b+ba)). We can see that, for symbol \emph{b}, the DFA has a transition to state \emph{2} from state \emph{1}. However, for symbol \emph{b}, the NFA has transitions to both state \emph{2} and \emph{3}. Independent of the rule and input stream, DFAs may only activate one state per symbol cycle. On the other hand, based on the rule and input stream, NFAs can activate multiple states while processing a symbol. Hence, for each symbol, NFAs need to determine the next active state(s) by scanning the adjacency list of the current active state(s) in linear time. As a result, in memory-bound CPU architectures, depending on the memory bandwidth, NFA's performance can get affected. On the other hand, Field Programming Gate Arrays (FPGAs) provide parallelism that allows NFA engines to process one symbol per clock cycle independent of the number of active states.\\ 
% If a regular language $L_1$ requires $m$ states and language $L_2$ requires $n$ states, then an NFA to represent $L_1 \cup L_2$ would require at most $m+n+1$ states \cite{holzer2003nondeterministic}, whereas an equivalent DFA might require as many as $m*n$ states \cite{yu1994state}. Previous works have shown that the memory requirement for implementing NFAs or DFAs into hardware is directly proportional to the size (state count) of these models \cite{kumar2006algorithms, hieu2013memory, xie2017reapr, becchi2009evaluating}.

% Therefore, it can be seen that there are a couple of aspects (size, performance) to consider before choosing between NFAs or DFAs as a computational model for pattern matching. \\
% Prior works \cite{yu2006fast, kumar2006algorithms} have studied the size of NFA and DFA on regex-based benchmarks, and Yu et al. stated that 20\% of the Snort \cite{roesch1999snort} DFAs suffer from exponential state growth. It is true that due to the power-set construction \cite{rabin1959finite} algorithm, NFA$\rightarrow$DFA conversion can result in an exponential state growth \cite{hopcroft2001introduction}. However, there exist algorithms \cite{hopcroft1971n, brzozowski1962canonical} to create a minimized DFA. Besides, Tabakov et al. \cite{tabakov2005experimental} performed a study on the randomly generated automata and illustrated that based on the automata structure, DFA states exhibit growth rate of the order \emph{polynomial to sub-exponential}. To the best of our knowledge, there has been no study that applies these DFA minimization algorithms on real-world automata benchmarks (Snort, Brill, ClamAV, Levenshtein, Hamming, Random Forest) and compares the size of NFA and DFA. Even though, the DFA size for these automata may be quite similar to the equivalent NFA, because of the lack of study in this regard, we do not have this data, yet. In this paper, we use DFA minimization algorithm and compares the size of the DFA to its equivalent NFA.\\
% DFAs have been widely used in memory-bound automata processing engine because of its sequential execution model \cite{RE2, yu2006fast}. On the other hand, due to NFA's non-deterministic parallel state activation behavior, FPGA-based architectures \cite{sidhu2001fast, xie2017reapr} use it extensively. Having said that, the state of the art CPU-based automata processing engine Hyperscan \cite{wang2019hyperscan} uses NFA as its computational model and Aho-Chorasick DFA model has been used \cite{hieu2013memory} to design FPGA-based automata processor. However, no existing research examines DFA and NFA's performance in relation to the FPGA and CPU-based automata processing engine. We present this performance analysis in this paper.\\
% Each automata benchmark is an aggregate of multiple rules, where each rule is used to describe a unique pattern. For example, the Snort \cite{roesch1999snort} benchmark in AutomataZoo \cite{wadden2018automatazoo} benchmark suite includes \emph{2,486} individual rules. The pattern matching applications are required to process each incoming input through all the individual rules to look for a match. However, depending on the input stream, all the rules might not get triggered evenly, as we will later see in this paper. There have been several works on dividing rules to multiple groups based on the automata size \cite{yu2006fast, becchi2009evaluating}. However, to the best of our knowledge, there has been no study on the frequency count of the triggered rules per input stream. As well as the automata size, a better understanding of the triggered rule frequency count would aid in the balanced distribution of rules among multiple groups. Moreover, a depiction of the triggered rule will help design high-performance pattern matching engines with optimized resource utilization. The most frequently triggered rule could be put in the FPGAs, and less frequently triggered ones could be placed in the CPU architecture.\\
% In this paper we systematically compare DFA vs. NFA  with respect to their size and performance. In summary, we made the following contributions:
% \begin{itemize}
%     \item We study the relative state count of NFA and minimized DFA both by keeping the rules separate as well as by incrementally merging the rules into one automaton. We used multiple benchmark classes for this study.
%     \begin{itemize}
%         \item Our findings from the individual rule state analysis suggests that, for benchmarks such as Snort, Brill, ClamAV, Hamming, Random Forest, and DotStar, minimized DFA state exhibit linear growth rate compared to the optimized NFA size. However, few of the rules from these benchmarks as well as all the rules of Levenshtein benchmark shows polynomial growth. (Section \ref{subsec:ind_state_count_analysis})
%         \item For multiple rules automata size, we see that minimized DFA exhibit exponential state growth for Hamming and Levenshtein benchmark. However, for Snort, Brill, DotStar and ClamAV minimized DFA's state grows linearly (Section \ref{subsec:multi_state_count_analysis}).
%     \end{itemize}
%     \item We identify the frequency count of the triggered rule per input cycle for regex-based benchmarks (Section \ref{subsec:active_rule}). The input files used for this experiment was taken from AutomataZoo benchmark suite. Our experiment shows that among 2,483 Snort rule, maximum 1,041 (41.92\%) and minimum 12 (0.5\%) rules are active at a time.
%     \item We study the  performance  of  NFA  and  DFA  on  the  FPGA,  versus state-of-the-art  CPU-based  automata  processing  engine,  Hyperscan (Section \ref{sec:perf_eval}). Findings from this study suggests that on spatial architectures, the choice of NFA over DFA is less important than the need to keep individual DFA rules separate and the ability to support parallel processing of a large  number  of  rules. 
% \end{itemize}
% Prior works \cite{becchi2007hybrid, yu2006fast} have shown that generating a DFA for a large set of distinct regular expressions can be infeasible as the DFA suffers from an exponential increase in the state. Besides, these studies are based on merging multiple regexes into one giant DFA. However, each benchmark consists of numerous regexes/rules. No work exists that performs an analysis on the DFA vs. NFA state count based on the individual rule.\\


% Linear time pattern matching in linear time has become an important research area. for its applicability in network security\cite{paxson1999bro, roesch1999snort, liu2011fast}, bioinformatics\cite{bo2018searching, roy2015discovering}, natural language processing \cite{zhou2015brill}, anti-virus\cite{ClamAV}, and machine learning \cite{tracy2016towards}.\\
% In summary, this paper made the following contribution:
% The motivation behind our work is to evaluate NFA and DFA as computational model on various paradigm of automata processing. In order to do that, we considered several property which we evaluated on the similar settings for both of these automata type.
% \begin{itemize}
% \item Three category of benchmarks, regex, synthetic etc.
% \item The very first property that we considered is, how the number of states of DFA compares to that of number states of an equivalent NFA. The reason behind this is, the performance of a computational model largely depends on the size of it. Even though previous works show that DFAs have much more higher number of states than the equivalent NFA, all of the works are based on the network intrusion detection benchmarks. However, to compare the size of DFA with its equivalent NFA, we used all the benchmarks from ANMLZoo and assessed the size of DFA vs NFA. Previous works suggest that complicated rules result in a larger DFA. Our hypotheses is if we merge several rules together, it will create a single complex rule. This single complex rule will generate a larger DFA. In order to prove this hypothesis, we ran following two experiments.
% \begin{itemize}
%     \item  We kept all the rules separate, and compared the states of minimized DFA with equivalent NFA. Our experiment shows that, except for Levenshtein, the number of states in DFA and the number of states in NFA are quite equal.
%     \item We incrementally started to merge rules and investigated how it affects the number of states in DFA. In this case, we saw that DFAs exhibit state explosion.
% \end{itemize}
% From the above two experiments, it can be safely asserted that in order to use DFA as a computational model for automata processing, we should keep each rule separate.
% \item The second property that we wanted to evaluate is, the performance of NFA vs DFA on spatial architecture. In this case, our hypothesis is, on spatial architectures, the question of NFA vs. DFA is less important than the need to keep individual DFA rules separate. The reason is, the rules can all be processed in parallel, and a large amount of memory-level parallelism is possible. In this scope, we ran an experiment using Grapefruit, on all the benchmarks of AutomataZoo. The experiment clearly indicates that, NFAs are efficient computation model while doing automata processing using FPGA.
% \item The third property that we considered is how these two computational model performs in CPU realm. For CPU processing, it's no wonder that parallel execution is a headache. Previous works have shown that, while doing automata processing using CPU, due to non-deterministic behavior of NFA, its performance deteriorates. However, our hypothesis is, as we are not merging rules, NFA model is not as unpredictable as it should be with all the rules mashed into a gigantic one. As a result, the performance of NFA and DFA should be comparable. Having said that, our experiment on Hyperscan, which is a CPU based architecture, shows that, if we keep each rule separated, NFA and DFA have somewhat same performance for almost all the benchmarks, except for Levenshtein. Due to the construction of Levenshtein automaton, DFA outperforms NFA. \\
% The rest of the paper is organized as follows.
% \end{itemize}


==> void/ReadingList.tex <==
\section{Reading List}
\subsection{Focus Papers}
\begin{enumerate}
    \small
    \item Tabakov  D,  Vardi  MY.   Experimental  evaluation  of  classical  automata constructions.  In:  International  Conference  on  Logic  for  Programming Artificial Intelligence and Reasoning. Springer; 2005. p. 396–411.
    \item Bo C, Dang V, Xie T, Wadden J, Stan M, Skadron K. Automata processing in reconfigurable architectures: In-the-cloud deployment, cross-platform evaluation, and fast symbol-only reconfiguration. ACM Transactions on Reconfigurable Technology and Systems (TRETS). 2019 May 17;12(2):1-25.
\end{enumerate}

\subsection{Background Readings}
\begin{enumerate}
    \small
    \item Hopcroft JE, Motwani R, Ullman JD.  Introduction to automata theory, languages, and computation.  ACM Sigact News. 2001;32(1):60–65.
    \item Rahimi  R,  Sadredini  E,  Stan  M,  Skadron  K.    Grapefruit:  An  Open-Source,  Full-Stack,  and  Customizable  Automata  Processing  on  FPGAs.   In:  2020  IEEE  28th  Annual  International  Symposium  on  Field-Programmable  Custom  Computing  Machines  (FCCM).  IEEE;  2020.  p.138–147.
    \item Wang   X,   Hong   Y,   Chang   H,   Park   K,   Langdale   G,   Hu   J,   et   al. Hyperscan:  a  fast  multi-pattern  regex  matcher  for  modern  CPUs.    In: 16th {USENIX} Symposium  on  Networked  Systems  Design  and  Implementation (\{NSDI\} 19); 2019. p. 631–648.
    \item Wadden J, Tracy T, Sadredini E, Wu L, Bo C, Du J, et al. AutomataZoo: A  modern  automata  processing  benchmark  suite. In:  2018  IEEE International Symposium on Workload Characterization (IISWC). IEEE;2018. p. 13–24.
    \item Becchi  M,  Crowley  P.   A  hybrid  finite  automaton  for  practical  deep packet inspection.  In: Proceedings of the 2007 ACM CoNEXT conference; 2007. p. 1–12.
\end{enumerate}


==> void/ResearchPlan.tex <==
\section{Research Plan}
In support of our proposed hypothesis, we outline the following research steps:
\begin{enumerate}[label=\textbf{S\arabic*}]
    \item \textbf{State Count Analysis:} In this step, we employ the DFA minimization algorithm and heuristic-based NFA optimization algorithm on several real-world benchmarks from the AutomataZoo. The objective of this step is to examine the state count and conversion complexity of the minimized DFA. Section \ref{sec:state_count_analysis} present the experimental setup and the evaluation strategy for this.   
    \item \textbf{Performance Analysis on FPGA (minimized DFA vs. optimized NFA):} Based on our insight from $S1$, we will synthesize the optimized NFA and minimized DFA on FPGA. Then we will present a study of the hardware utilization and performance of both the computation model. This step is crucial for proving or disproving our hypothesis $H1$. We present the experimental setup and evaluation strategy for this experiment in Section \ref{sec:grpfrt}.  
    \item \textbf{Performance Analysis (CPU vs. FPGA):} We will present a performance comparison for the state-of-the-art CPU-based automata processing engine and the state-of-the-art FPGA-based automata processing engine to support our claim made in hypothesis $H2$. Our detailed approach for this step can be found in section \ref{sec:perf_eval}.
\end{enumerate}
As a part of the feasibility justification of this proposal, we have mostly finished $S1$. Figure \ref{fig:statecomp} \& \ref{fig:statecompmulti} exhibits the visual representation of our findings so far. Besides, we have a few data for $S3$ (Table \ref{tab:hps_grp} presents the result obtained so far). \\
Our remaining tasks include: 
\begin{itemize}
    \item For $S1$, we intend to analyze further the cases where the state count for mDFA and equivalent optimized NFA don't keep up. 
    \item Performance Analysis on FPGA (minimized DFA vs. optimized NFA). 
    \item Expanding $S3$ across all the benchmarks from the AutomataZoo benchmark suite.
    \item Verifying the accuracy of the CPU throughput.
\end{itemize}
 
